Effect of Phonons and Impurities on the Quantum Transport in XXZ Spin-Chains

Numerical and analytic results have been used to characterize quantum transport in spin chains, showing the existence of both ballistic and diffusive motion. Experiments have shown that heat transfer is surprisingly always diffusive. The scattering from phonons and impurities have been postulated to be the two factors critical in causing the diffusive transport. In this work, we evaluate the transport process by incorporating a bath of phonons and impurities in order to understand the role played by each of the factors. While methods like time-dependent density matrix renormalization group (tDMRG) can be used to simulate isolated spin chains, the coupling with phonons make simulations significantly more challenging. The recently developed multisite tensor network path integral (MS-TNPI) method builds a framework for simulating the dynamics in extended open quantum systems by combining ideas from tDMRG and Feynman-Vernon influence functional. This MS-TNPI is used to characterize dynamics in open, extended quantum systems. Simulations are done with the commonly used sub-Ohmic, Ohmic and super-Ohmic spectral densities describing the phononic bath. We show that while the transport in presence of impurities eventually becomes diffusive, the exact details are dependent on the specifics of the interactions and amount of impurities. In contrast, the presence of a bath makes the transport diffusive irrespective of the parameters characterizing the bath.

==> bibexport.bib-save-2022.07.01_14.06.00 <==


@article{gopalakrishnanAnomalousRelaxationHightemperature2019,
  author =        {Gopalakrishnan, Sarang and Vasseur, Romain and
                   {Brayden Ware}},
  journal =       {Proceedings of the National Academy of Sciences},
  number =        {33},
  pages =         {16250--16255},
  title =         {Anomalous Relaxation and the High-Temperature
                   Structure Factor of {{XXZ}} Spin Chains},
  volume =        {116},
  year =          {2019},
  abstract =      {The XXZ model is a canonical model of quantum
                   magnetism. In one dimension, this model is integrable
                   and has ballistically moving quasiparticles; thus,
                   energy spreads ballistically, but, surprisingly, spin
                   transport can be diffusive or superdiffusive. Here,
                   we show that spin transport is even richer in the
                   presence of a magnetic field: Some fraction of the
                   spin moves out ballistically, but the dynamical
                   spin-structure factor decays with an anomalous,
                   continuously varying exponent. A hitherto-unnoticed
                   phase transition takes place at finite fields,
                   separating ballistic from subballistic decay of local
                   correlations. We analytically derive these results
                   using generalized hydrodynamics and support our
                   findings numerically. These anomalous exponents can
                   readily be measured via the frequency and wavevector
                   dependence of the spin conductivity. We compute the
                   spin-structure factor of XXZ spin chains in the
                   Heisenberg and gapped (Ising) regimes in the
                   high-temperature limit for nonzero magnetization,
                   within the framework of generalized hydrodynamics,
                   including diffusive corrections. The structure factor
                   shows a hierarchy of timescales in the gapped phase,
                   owing to s-spin magnon bound states (``strings'') of
                   various sizes. Although short strings move
                   ballistically, long strings move primarily
                   diffusively as a result of their collisions with
                   short strings. The interplay between these effects
                   gives rise to anomalous power-law decay of the
                   spin-structure factor, with continuously varying
                   exponents, at any fixed separation in the late-time
                   limit. We elucidate the cross-over to diffusion (in
                   the gapped phase) and to superdiffusion (at the
                   isotropic point) in the half-filling limit. We verify
                   our results via extensive matrix product operator
                   calculations.},
  doi =           {10.1073/pnas.1906914116},
}

@article{prosenOpenXXZSpin2011,
  author =        {Prosen, Tomaz},
  journal =       {Physical Review Letters},
  month =         may,
  number =        {21},
  pages =         {217206},
  publisher =     {{American Physical Society}},
  title =         {Open {{XXZ Spin Chain}}: {{Nonequilibrium Steady
                   State}} and a {{Strict Bound}} on {{Ballistic
                   Transport}}},
  volume =        {106},
  year =          {2011},
  doi =           {10.1103/PhysRevLett.106.217206},
}

@article{prosenExactNonequilibriumSteady2011,
  author =        {Prosen, Tom{\v a}z{\v z}},
  journal =       {Phys. Rev. Lett.},
  month =         sep,
  number =        {13},
  pages =         {137201},
  publisher =     {{American Physical Society}},
  title =         {Exact Nonequilibrium Steady State of a Strongly
                   Driven Open {{XXZ}} Chain},
  volume =        {107},
  year =          {2011},
  doi =           {10.1103/PhysRevLett.107.137201},
}

@article{cornelissenLongdistanceTransportMagnon2015,
  author =        {Cornelissen, L. J. and Liu, J. and Duine, R. A. and
                   Youssef, J. Ben and {van Wees}, B. J.},
  journal =       {Nature Physics},
  month =         dec,
  number =        {12},
  pages =         {1022--1026},
  title =         {Long-Distance Transport of Magnon Spin Information in
                   a Magnetic Insulator at Room~Temperature},
  volume =        {11},
  year =          {2015},
  abstract =      {Although electron motion is prohibited in magnetic
                   insulators, the electron spin can be transported by
                   magnons. Such magnons, generated and detected using
                   all-electrical methods, are now shown to travel
                   micrometre distances at room temperature.},
  doi =           {10.1038/nphys3465},
  issn =          {1745-2481},
}

@article{kuklovCounterflowSuperfluidityTwospecies2003,
  author =        {Kuklov, A. B. and Svistunov, B. V.},
  journal =       {Phys. Rev. Lett.},
  month =         mar,
  number =        {10},
  pages =         {100401},
  publisher =     {{American Physical Society}},
  title =         {Counterflow Superfluidity of Two-Species Ultracold
                   Atoms in a Commensurate Optical Lattice},
  volume =        {90},
  year =          {2003},
  doi =           {10.1103/PhysRevLett.90.100401},
}

@article{mandelCoherentTransportNeutral2003,
  author =        {Mandel, Olaf and Greiner, Markus and Widera, Artur and
                   Rom, Tim and H{\"a}nsch, Theodor W. and
                   Bloch, Immanuel},
  journal =       {Phys. Rev. Lett.},
  month =         jul,
  number =        {1},
  pages =         {010407},
  publisher =     {{American Physical Society}},
  title =         {Coherent Transport of Neutral Atoms in Spin-Dependent
                   Optical Lattice Potentials},
  volume =        {91},
  year =          {2003},
  doi =           {10.1103/PhysRevLett.91.010407},
}

@article{castro-alvaredoEmergentHydrodynamicsIntegrable2016,
  author =        {{Castro-Alvaredo}, Olalla A. and Doyon, Benjamin and
                   Yoshimura, Takato},
  journal =       {Phys. Rev. X},
  month =         dec,
  number =        {4},
  pages =         {041065},
  publisher =     {{American Physical Society}},
  title =         {Emergent Hydrodynamics in Integrable Quantum Systems
                   out of Equilibrium},
  volume =        {6},
  year =          {2016},
  doi =           {10.1103/PhysRevX.6.041065},
}

@article{bertiniTransportOutofequilibriumXXZ2016,
  author =        {Bertini, Bruno and Collura, Mario and
                   De Nardis, Jacopo and Fagotti, Maurizio},
  journal =       {Phys. Rev. Lett.},
  month =         nov,
  number =        {20},
  pages =         {207201},
  publisher =     {{American Physical Society}},
  title =         {Transport in Out-of-Equilibrium {{XXZ}} Chains:
                   {{Exact}} Profiles of Charges and Currents},
  volume =        {117},
  year =          {2016},
  doi =           {10.1103/PhysRevLett.117.207201},
}

@article{ljubotinaSpinDiffusionInhomogeneous2017,
  author =        {Ljubotina, Marko and {\v Z}nidari{\v c}, Marko and
                   Prosen, Toma{\v z}},
  journal =       {Nature Communications},
  month =         jul,
  number =        {1},
  pages =         {16117},
  title =         {Spin Diffusion from an Inhomogeneous Quench in an
                   Integrable System},
  volume =        {8},
  year =          {2017},
  abstract =      {Generalized hydrodynamics predicts universal
                   ballistic transport in integrable lattice systems
                   when prepared in generic inhomogeneous initial
                   states. However, the ballistic contribution to
                   transport can vanish in systems with additional
                   discrete symmetries. Here we perform large scale
                   numerical simulations of spin dynamics in the
                   anisotropic Heisenberg XXZ spin 1/2 chain starting
                   from an inhomogeneous mixed initial state which is
                   symmetric with respect to a combination of spin
                   reversal and spatial reflection. In the isotropic and
                   easy-axis regimes we find non-ballistic spin
                   transport which we analyse in detail in terms of
                   scaling exponents of the transported magnetization
                   and scaling profiles of the spin density. While in
                   the easy-axis regime we find accurate evidence of
                   normal diffusion, the spin transport in the isotropic
                   case is clearly super-diffusive, with the scaling
                   exponent very close to 2/3, but with universal
                   scaling dynamics which obeys the diffusion equation
                   in nonlinearly scaled time.},
  doi =           {10.1038/ncomms16117},
  issn =          {2041-1723},
}

@article{whiteRealTimeEvolutionUsing2004,
  author =        {White, Steven R. and Feiguin, Adrian E.},
  journal =       {Physical Review Letters},
  number =        {7},
  pages =         {076401},
  publisher =     {{American Physical Society (APS)}},
  title =         {Real-{{Time Evolution Using}} the {{Density Matrix
                   Renormalization Group}}},
  volume =        {93},
  year =          {2004},
  abstract =      {We describe an extension to the density matrix
                   renormalization group method incorporating real-time
                   evolution. Its application to transport problems in
                   systems out of equilibrium and frequency dependent
                   correlation functions is discussed and illustrated in
                   several examples. We simulate a scattering process in
                   a spin chain which generates a spatially nonlocal
                   entangled wave function.},
  doi =           {10.1103/physrevlett.93.076401},
  isbn =          {0031-9007},
}

@article{schollwockDensitymatrixRenormalizationGroup2011a,
  author =        {Schollw{\"o}ck, Ulrich},
  journal =       {Annals of Physics},
  number =        {1},
  pages =         {96--192},
  publisher =     {{Elsevier BV}},
  title =         {The Density-Matrix Renormalization Group in the Age
                   of Matrix Product States},
  volume =        {326},
  year =          {2011},
  abstract =      {The density-matrix renormalization group method
                   (DMRG) has established itself over the last decade as
                   the leading method for the simulation of the statics
                   and dynamics of one-dimensional strongly correlated
                   quantum lattice systems. In the further development
                   of the method, the realization that DMRG operates on
                   a highly interesting class of quantum states,
                   so-called matrix product states (MPS), has allowed a
                   much deeper understanding of the inner structure of
                   the DMRG method, its further potential and its
                   limitations. In this paper, I want to give a detailed
                   exposition of current DMRG thinking in the MPS
                   language in order to make the advisable
                   implementation of the family of DMRG algorithms in
                   exclusively MPS terms transparent. I then move on to
                   discuss some directions of potentially fruitful
                   further algorithmic development: while DMRG is a very
                   mature method by now, I still see potential for
                   further improvements, as exemplified by a number of
                   recently introduced algorithms.},
  doi =           {10.1016/j.aop.2010.09.012},
  isbn =          {0003-4916},
}

@article{vidalEfficientSimulationOneDimensional2004,
  author =        {Vidal, Guifr{\'e}},
  journal =       {Physical Review Letters},
  month =         jul,
  number =        {4},
  pages =         {040502},
  publisher =     {{American Physical Society}},
  title =         {Efficient {{Simulation}} of {{One-Dimensional Quantum
                   Many-Body Systems}}},
  volume =        {93},
  year =          {2004},
  doi =           {10.1103/PhysRevLett.93.040502},
}

@article{paeckelTimeevolutionMethodsMatrixproduct2019,
  author =        {Paeckel, Sebastian and K{\"o}hler, Thomas and
                   Swoboda, Andreas and Manmana, Salvatore R. and
                   Schollw{\"o}ck, Ulrich and Hubig, Claudius},
  journal =       {Annals of Physics},
  pages =         {167998},
  publisher =     {{Elsevier BV}},
  title =         {Time-Evolution Methods for Matrix-Product States},
  volume =        {411},
  year =          {2019},
  abstract =      {Matrix-product states have become the de facto
                   standard for the representation of one-dimensional
                   quantum many body states. During the last few years,
                   numerous new methods have been introduced to evaluate
                   the time evolution of a matrix-product state. Here,
                   we will review and summarize the recent work on this
                   topic as applied to finite quantum systems. We will
                   explain and compare the different methods available
                   to construct a time-evolved matrix-product state,
                   namely the time-evolving block decimation, the MPO
                   WI,II method, the global Krylov method, the local
                   Krylov method and the one- and two-site
                   time-dependent variational principle. We will also
                   apply these methods to four different representative
                   examples of current problem settings in condensed
                   matter physics.},
  doi =           {10.1016/j.aop.2019.167998},
  isbn =          {0003-4916},
}

@article{gobertRealtimeDynamicsSpin2005,
  author =        {Gobert, Dominique and Kollath, Corinna and
                   Schollw{\"o}ck, Ulrich and Sch{\"u}tz, Gunter},
  journal =       {Phys. Rev. E},
  month =         mar,
  number =        {3},
  pages =         {036102},
  publisher =     {{American Physical Society}},
  title =         {Real-Time Dynamics in Spin-{$\frac{1}{2}$} Chains
                   with Adaptive Time-Dependent Density Matrix
                   Renormalization Group},
  volume =        {71},
  year =          {2005},
  doi =           {10.1103/PhysRevE.71.036102},
}

@article{hlubekSpinonHeatTransport2012,
  author =        {Hlubek, N and Zotos, X and Singh, S and
                   {Saint-Martin}, R and Revcolevschi, A and
                   B{\"u}chner, B and Hess, C},
  journal =       {Journal of Statistical Mechanics: Theory and
                   Experiment},
  month =         mar,
  number =        {03},
  pages =         {P03006},
  publisher =     {{IOP Publishing}},
  title =         {Spinon Heat Transport and Spin\textendash Phonon
                   Interaction in the Spin-1/2 {{Heisenberg}} Chain
                   Cuprates {{Sr}}{$_{2}$}{{CuO}}{$_3$} and
                   {{SrCuO}}{$_{2}$}},
  volume =        {2012},
  year =          {2012},
  abstract =      {We have investigated the thermal conductivity
                   {$\kappa$}mag of high-purity single crystals of the
                   spin chain compound Sr2CuO3, which is considered an
                   excellent realization of the one-dimensional spin-1/2
                   antiferromagnetic Heisenberg model. We find that the
                   spinon heat conductivity {$\kappa$}mag is strongly
                   enhanced as compared to previous results obtained on
                   samples with lower chemical purity. The analysis of
                   {$\kappa$}mag allows the computation of the spinon
                   mean free path lmag as a function of temperature. At
                   low temperature we find lmag {$\sim$} 0.5 \textmu m,
                   corresponding to more than 1200 chain unit cells.
                   Upon increasing the temperature, the mean free path
                   decreases strongly and approaches an exponential
                   decay {$\sim$} (1/T)exp(Tu*/T), which is
                   characteristic for Umklapp processes with the energy
                   scale kBTu*. Based on Matthiessen's rule we decompose
                   lmag into a temperature-independent spinon\textendash
                   defect scattering length l0 and a
                   temperature-dependent spinon\textendash phonon
                   scattering length lsp(T). By comparing lmag(T) of
                   Sr2CuO3 with that of SrCuO2, we show that the
                   spin\textendash phonon interaction, as expressed by
                   lsp, is practically the same in both systems. The
                   comparison of the empirically derived lsp with model
                   calculations for the spin\textendash phonon
                   interaction of the one-dimensional spin-1/2 XY model
                   yields reasonable agreement with the experimental
                   data.},
  doi =           {10.1088/1742-5468/2012/03/p03006},
}

@article{haegemanTimeDependentVariationalPrinciple2011,
  author =        {Haegeman, Jutho and Cirac, J. Ignacio and
                   Osborne, Tobias J. and Pi{\v z}orn, Iztok and
                   Verschelde, Henri and Verstraete, Frank},
  journal =       {Physical Review Letters},
  number =        {7},
  pages =         {070601},
  publisher =     {{American Physical Society}},
  title =         {Time-{{Dependent Variational Principle}} for
                   {{Quantum Lattices}}},
  volume =        {107},
  year =          {2011},
  doi =           {10.1103/PhysRevLett.107.070601},
}

@article{haegemanUnifyingTimeEvolution2016,
  author =        {Haegeman, Jutho and Lubich, Christian and
                   Oseledets, Ivan and Vandereycken, Bart and
                   Verstraete, Frank},
  journal =       {Phys. Rev. B},
  month =         oct,
  number =        {16},
  pages =         {165116},
  publisher =     {{American Physical Society}},
  title =         {Unifying Time Evolution and Optimization with Matrix
                   Product States},
  volume =        {94},
  year =          {2016},
  doi =           {10.1103/PhysRevB.94.165116},
}

@article{klossTimedependentVariationalPrinciple2018,
  author =        {Kloss, Benedikt and Lev, Yevgeny Bar and
                   Reichman, David},
  journal =       {Phys. Rev. B},
  month =         jan,
  number =        {2},
  pages =         {024307},
  publisher =     {{American Physical Society}},
  title =         {Time-Dependent Variational Principle in
                   Matrix-Product State Manifolds: {{Pitfalls}} and
                   Potential},
  volume =        {97},
  year =          {2018},
  doi =           {10.1103/PhysRevB.97.024307},
}

@article{gotoPerformanceTimedependentVariational2019,
  author =        {Goto, Shimpei and Danshita, Ippei},
  journal =       {Phys. Rev. B},
  month =         feb,
  number =        {5},
  pages =         {054307},
  publisher =     {{American Physical Society}},
  title =         {Performance of the Time-Dependent Variational
                   Principle for Matrix Product States in the Long-Time
                   Evolution of a Pure State},
  volume =        {99},
  year =          {2019},
  doi =           {10.1103/PhysRevB.99.054307},
}

@article{feynmanTheoryGeneralQuantum1963,
  author =        {Feynman, R P and Vernon, F L},
  journal =       {Annals of Physics},
  pages =         {118--173},
  publisher =     {{Elsevier BV}},
  title =         {The Theory of a General Quantum System Interacting
                   with a Linear Dissipative System},
  volume =        {24},
  year =          {1963},
  abstract =      {A formalism has been developed, using Feynman's
                   space-time formulation of nonrelativistic quantum
                   mechanics whereby the behavior of a system of
                   interest, which is coupled to other external quantum
                   systems, may be calculated in terms of its own
                   variables only. It is shown that the effect of the
                   external systems in such a formalism can always be
                   included in a general class of functionals (influence
                   functionals) of the coordinates of the system only.
                   The properties of influence functionals for general
                   systems are examined. Then, specific forms of
                   influence functionals representing the effect of
                   definite and random classical forces, linear
                   dissipative systems at finite temperatures, and
                   combinations of these are analyzed in detail. The
                   linear system analysis is first done for perfectly
                   linear systems composed of combinations of harmonic
                   oscillators, loss being introduced by continuous
                   distributions of oscillators. Then approximately
                   linear systems and restrictions necessary for the
                   linear behavior are considered. Influence functionals
                   for all linear systems are shown to have the same
                   form in terms of their classical response functions.
                   In addition, a fluctuation-dissipation theorem is
                   derived relating temperature and dissipation of the
                   linear system to a fluctuating classical potential
                   acting on the system of interest which reduces to the
                   Nyquist-Johnson relation for noise in the case of
                   electric circuits. Sample calculations of transition
                   probabilities for the spontaneous emission of an atom
                   in free space and in a cavity are made. Finally, a
                   theorem is proved showing that within the
                   requirements of linearity all sources of noise or
                   quantum fluctuation introduced by maser-type
                   amplification devices are accounted for by a
                   classical calculation of the characteristics of the
                   maser.},
  doi =           {10.1016/0003-4916(63)90068-x},
  isbn =          {0003-4916},
}

@article{strathearnEfficientNonMarkovianQuantum2018,
  author =        {Strathearn, A. and Kirton, P. and Kilda, D. and
                   Keeling, J. and Lovett, B. W.},
  journal =       {Nature Communications},
  number =        {1},
  pages =         {1---9},
  publisher =     {{Springer Science and Business Media LLC}},
  title =         {Efficient Non-{{Markovian}} Quantum Dynamics Using
                   Time-Evolving Matrix Product Operators},
  volume =        {9},
  year =          {2018},
  abstract =      {In order to model realistic quantum devices it is
                   necessary to simulate quantum systems strongly
                   coupled to their environment. To date, most
                   understanding of open quantum systems is restricted
                   either to weak system\textendash bath couplings or to
                   special cases where specific numerical techniques
                   become effective. Here we present a general and yet
                   exact numerical approach that efficiently describes
                   the time evolution of a quantum system coupled to a
                   non-Markovian harmonic environment. Our method relies
                   on expressing the system state and its propagator as
                   a matrix product state and operator, respectively,
                   and using a singular value decomposition to compress
                   the description of the state as time evolves. We
                   demonstrate the power and flexibility of our approach
                   by numerically identifying the localisation
                   transition of the Ohmic spin-boson model, and
                   considering a model with widely separated
                   environmental timescales arising for a pair of spins
                   embedded in a common environment.},
  doi =           {10.1038/s41467-018-05617-3},
  isbn =          {2041-1723},
}

@article{jorgensenExploitingCausalTensor2019,
  author =        {J{\o}rgensen, Mathias R. and Pollock, Felix A.},
  journal =       {Physical Review Letters},
  number =        {24},
  pages =         {240602},
  publisher =     {{American Physical Society (APS)}},
  title =         {Exploiting the {{Causal Tensor Network Structure}} of
                   {{Quantum Processes}} to {{Efficiently Simulate
                   Non-Markovian Path Integrals}}},
  volume =        {123},
  year =          {2019},
  abstract =      {In the path integral formulation of the evolution of
                   an open quantum system coupled to a Gaussian,
                   noninteracting environment, the dynamical
                   contribution of the latter is encoded in an object
                   called the influence functional. Here, we relate the
                   influence functional to the process tensor\textemdash
                   a more general representation of a quantum stochastic
                   process\textemdash describing the evolution. Then, we
                   use this connection to motivate a tensor network
                   algorithm for the simulation of multitime
                   correlations in open systems, building on recent work
                   where the influence functional is represented in
                   terms of time evolving matrix product operators. By
                   exploiting the symmetries of the influence
                   functional, we are able to use our algorithm to
                   achieve orders-of-magnitude improvement in the
                   efficiency of the resulting numerical simulation. Our
                   improved algorithm is then applied to compute exact
                   phonon emission spectra for the spin-boson model with
                   strong coupling, demonstrating a significant
                   divergence from spectra derived under commonly used
                   assumptions of memorylessness.},
  doi =           {10.1103/physrevlett.123.240602},
  isbn =          {0031-9007},
}

@article{boseTensorNetworkRepresentation2021,
  author =        {Bose, Amartya and Walters, Peter L.},
  journal =       {arXiv pre-print server},
  title =         {A Tensor Network Representation of Path Integrals:
                   {{Implementation}} and Analysis},
  year =          {2021},
  abstract =      {Tensors with finite correlation afford very compact
                   tensor network representations. A novel tensor
                   network-based decomposition of real-time path
                   integral simulations involving Feynman-Vernon
                   influence functional is introduced. In this tensor
                   network path integral (TNPI) technique, the
                   finitetemporarily non-local interactions introduced
                   by the influence functional can be captured very
                   effi-ciently using matrix product state
                   representation for the path-dependent Green's
                   function (PDGF). We illustrate this particular TNPI
                   method through various realistic examples, including
                   a chargetransfer reaction and an exciton transfer in
                   a dimer. We also show how it is readily applied to
                   systems with greater than two states. PDGF-TNPI
                   utilizes the symmetries of the problem, leading to
                   accelerated convergence and dramatic reductions of
                   computational effort. We also introduce anapproximate
                   method that speeds up propagation beyond the
                   non-local memory length. Further-more, the structure
                   imposed by the tensor network representation of the
                   PDGF naturally suggests other factorizations that
                   make simulations for extended systems more efficient.
                   These factorizations would be the subject of future
                   explorations. The flexibility of the PDGF-TNPI
                   framework makesit a promising new addition to the
                   family of path integral methods for non-equilibrium
                   quantum dynamics.},
  doi =           {arxiv:2106.12523},
}

@article{bosePairwiseConnectedTensor2022,
  author =        {Bose, Amartya},
  journal =       {Physical Review B},
  number =        {2},
  pages =         {024309},
  publisher =     {{American Physical Society}},
  title =         {Pairwise Connected Tensor Network Representation of
                   Path Integrals},
  volume =        {105},
  year =          {2022},
  doi =           {10.1103/PhysRevB.105.024309},
}

@article{boseMultisiteDecompositionTensor2022,
  author =        {Bose, Amartya and Walters, Peter L.},
  journal =       {The Journal of Chemical Physics},
  number =        {2},
  pages =         {024101},
  title =         {A Multisite Decomposition of the Tensor Network Path
                   Integrals},
  volume =        {156},
  year =          {2022},
  abstract =      {Tensor network decompositions of path integrals for
                   simulating open quantum systems have recently been
                   proven to be useful. However, these methods scale
                   exponentially with the system size. This makes it
                   challenging to simulate the non-equilibrium dynamics
                   of extended quantum systems coupled with local
                   dissipative environments. In this work, we extend the
                   tensor network path integral (TNPI) framework to
                   efficiently simulate such extended systems. The
                   Feynman\textendash Vernon influence functional is a
                   popular approach used to account for the effect of
                   environments on the dynamics of the system. In order
                   to facilitate the incorporation of the influence
                   functional into a multisite framework (MS-TNPI), we
                   combine a matrix product state (MPS) decomposition of
                   the reduced density tensor of the system along the
                   sites with a corresponding tensor network
                   representation of the time axis to construct an
                   efficient 2D tensor network. The 2D MS-TNPI network,
                   when contracted, yields the time-dependent reduced
                   density tensor of the extended system as an MPS. The
                   algorithm presented is independent of the system
                   Hamiltonian. We outline an iteration scheme to take
                   the simulation beyond the non-Markovian memory
                   introduced by solvents. Applications to spin chains
                   coupled to local harmonic baths are presented; we
                   consider the Ising, XXZ, and Heisenberg models,
                   demonstrating that the presence of local environments
                   can often dissipate the entanglement between the
                   sites. We discuss three factors causing the system to
                   transition from a coherent oscillatory dynamics to a
                   fully incoherent dynamics. The MS-TNPI method is
                   useful for studying a variety of extended quantum
                   systems coupled with solvents.},
  doi =           {10.1063/5.0073234},
}

@article{boseTensorNetworkPath2022,
  author =        {Bose, Amartya and Walters, Peter L.},
  journal =       {arXiv pre-print server},
  title =         {Tensor Network Path Integral Study of Dynamics in
                   {{B850 LH2}} Ring with Atomistically Derived
                   Vibrations},
  year =          {2022},
  doi =           {arXiv:2202.05350},
}

@article{makriTensorPropagatorIterativeI1995,
  author =        {Makri, Nancy and Makarov, Dmitrii E.},
  journal =       {The Journal of Chemical Physics},
  number =        {11},
  pages =         {4600--4610},
  publisher =     {{AIP Publishing}},
  title =         {Tensor Propagator for Iterative Quantum Time
                   Evolution of Reduced Density Matrices. {{I}}.
                   {{Theory}}},
  volume =        {102},
  year =          {1995},
  abstract =      {For common condensed phase problems described by a
                   low-dimensional system coupled to a harmonic bath,
                   Feynman's path integral formulation of time-dependent
                   quantum mechanics leads to expressions for the
                   reduced density matrix of the system where the
                   effects of the harmonic environment enter through an
                   influence functional that is nonlocal in time. In a
                   recent Letter [Chem. Phys. Lett. 221, 482 (1994)], we
                   demonstrated that the range of the nonlocal
                   interactions is finite even at zero temperature, such
                   that the nonlocal kernel extends over only a few time
                   steps if the path integral is expressed in terms of
                   accurate quasiadiabatic propagators. This feature
                   arises from disruption of phase coherence in
                   macroscopic environments and leads to Markovian
                   dynamics for an augmented reduced density tensor,
                   permitting iterative time evolution schemes. In the
                   present paper we analyze the structure and properties
                   of the relevant tensor propagator. Specifically, we
                   show that the tensor multiplication scheme rigorously
                   conserves the trace of the reduced density matrix,
                   and that in cases of short-range nonlocality it leads
                   to Redfield-type equations which are correct to all
                   orders in perturbation theory and which take into
                   account memory effects. We also argue that a simple
                   eigenvector analysis reveals (without actual
                   iteration) the nature of the dynamics and of the
                   equilibrium state, and directly yields quantum
                   reaction or relaxation rates.},
  doi =           {10.1063/1.469508},
  isbn =          {0021-9606},
}

@article{makriTensorPropagatorIterativeII1995,
  author =        {Makri, Nancy and Makarov, Dmitrii E.},
  journal =       {The Journal of Chemical Physics},
  number =        {11},
  pages =         {4611--4618},
  publisher =     {{AIP Publishing}},
  title =         {Tensor Propagator for Iterative Quantum Time
                   Evolution of Reduced Density Matrices. {{II}}.
                   {{Numerical}} Methodology},
  volume =        {102},
  year =          {1995},
  abstract =      {In a recent Letter [Chem. Phys. Lett. 221, 482
                   (1994)], we demonstrated that the dynamics of reduced
                   density matrices for systems in contact with
                   dissipative harmonic environments can be obtained in
                   an iterative fashion by multiplication of a
                   propagator tensor. The feasibility of iterative
                   procedures in reduced dimension spaces arises from
                   intrinsic features of the dissipative influence
                   functional in Feynman's path integral formulation of
                   quantum dynamics. Specifically, the continuum of
                   frequencies characteristic of broad condensed phase
                   spectra disrupts phase coherence to a large extent,
                   such that the dynamics of an augmented reduced
                   density tensor becomes Markovian. In a preceding
                   article [J. Chem. Phys. 102, 4600 (1995)] we examined
                   in detail the formal properties of the tensor
                   propagator. In the present paper we show that the
                   tensor propagator can be further decomposed into a
                   product of small rank tensors, resulting in an
                   extremely simple and efficient numerical scheme that
                   scales almost linearly with the dimension of the
                   augmented reduced density tensor. Numerical
                   application to a model electron transfer reaction is
                   presented.},
  doi =           {10.1063/1.469509},
  isbn =          {0021-9606},
}

